A Markov Decision Process for Response-Adaptive Randomization in Clinical Trials

In clinical trials, response-adaptive randomization (RAR) has the appealing ability to assign more subjects to better-performing treatments based on interim results. The traditional RAR strategy alters the randomization ratio on a patient-by-patient basis; this has been heavily criticized for bias due to time-trends. An alternate approach is blocked RAR, which groups patients together in blocks and recomputes the randomization ratio in a block-wise fashion; the final analysis is then stratified by block. However, the typical blocked RAR design divides patients into equal-sized blocks, which is not generally optimal. This paper presents TrialMDP, an algorithm that designs two-armed blocked RAR clinical trials. Our method differs from past approaches in that it optimizes the size and number of blocks as well as their treatment allocations. That is, the algorithm yields a policy that adaptively chooses the size and composition of the next block, based on results seen up to that point in the trial. TrialMDP is related to past works that compute optimal trial designs via dynamic programming. The algorithm maximizes a utility function balancing (i) statistical power, (ii) patient outcomes, and (iii) the number of blocks. We show that it attains significant improvements in utility over a suite of baseline designs, and gives useful control over the tradeoff between statistical power and patient outcomes. It is well suited for small trials that assign high cost to failures. We provide TrialMDP as an R package on GitHub: https://github.com/dpmerrell/TrialMDP

==> figures_tables.tex <==


\begin{figure}
    \centering
    \includegraphics[scale=0.7]{figures/contingency_table.png}
    \hspace{1em}
    \includegraphics[scale=0.7]{figures/history.png}\\
    (A) \hspace{2.75in} (B)
    \caption{(A) Contingency table notation. (B) Trial history notation. A history $h$ is a sequence of cumulative contingency tables, $(s_0, \ldots, s_K)$. A subscript $h_k$ indicates a history's $k$th \emph{suffix}.}
    \label{fig:contingency}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{figures/state_space.png}
    \includegraphics[scale=0.7]{figures/transitions.png}\\
    (A) \hspace{2.5in} (B)
    \caption{(A) State space $S$. At any point, the state of the trial is summarized by its contingency table. We can order the set of all contingency tables by their sums, $T$. The trial begins with the empty table in $S_0$; the trial ends when it reaches a state in $S_N$ (in this example $N{=}100$). 
    (B) Transition distribution. In this example, current state $s$ and action $a{=}(60,0.7)$ induce a distribution $s^\prime \sim t(s,a)$ for the next state. 
    The next state necessarily has $\underline{T} {=} 144 {=} 84 + 60$. 
    Its entries are governed by Beta-Binomial distributions, parameterized by the entries of the current contingency table. %Given the current state $s$ and chosen action $a$, the trial's next state $s^\prime$ is randomly distributed according to $t(s,a)$, the transition distribution.
    }
    \label{fig:states}
\end{figure}

\newcommand{\vnew}{$v_{\text{new}}$}
\begin{figure}
    \centering

    \begingroup
    \begin{minipage}{0.5\linewidth}
    \begin{algorithm}[H]
    \caption{\textsc{TrialMDP}}
    \begin{algorithmic}[1]
    \setlength{\baselineskip}{12pt}
    \Procedure{MainLoop}{$N, \lambda_F, \lambda_K$}
      \State initialize tables U, A
      \For{ $s \in S_{N}$ }
        \State U[s] = 0
      \EndFor
      \For{ $s \notin S_{N}$ }
        \State U[$s$] $ = -\infty$
        \For{ $a \in \mathcal{A}_s$ }
          %\State initialize struct $v$
          \State $\text{u} = 0$
          \For{$(p, s^\prime) \in t(s, a)$}
            \State $\text{u} {\pluseq} p {\cdot} \big\{ R(a, s^\prime, N, \lambda_F, \lambda_K)$ 
            \State \hfill ${+} \text{U}[s^\prime] \big\}$
          \EndFor
          \If{u $>$ U[$s$]}
            \State U[s] = u; A[s] = $a$
          \EndIf
        \EndFor
      \EndFor
      \State \Return U, A
    \EndProcedure
    %\end{spacing}
    \end{algorithmic}
    \end{algorithm}
    \end{minipage}
    \begin{minipage}{0.45\linewidth}
    %\begin{algorithm}[H]
    \begin{algorithmic}
    \setlength{\baselineskip}{12pt}
    \Function{$R$}{$a,s^\prime, N, \lambda_F, \lambda_K$}
        \State $r = 0$ 
        \State $w = a.N_A \cdot a.N_B / (a.N_A + a.N_B) $
        \State $\hat{p}_A = (s^\prime.n_A {+} 1)/ (s^\prime.N_A {+} 2)$
        \State $\hat{p}_B = (s^\prime.n_B {+} 1)/ (s^\prime.N_B {+} 2)$
        \State $\hat{q}_A = 1 - \hat{p}_A$
        \State $\hat{q}_B = 1 - \hat{p}_B$
        \State $r \pluseq 4 \cdot w / (N {\cdot} (\hat{p}_A {+} \hat{p}_B) (\hat{q}_A {+} \hat{q}_B))$
        \If{ $s^\prime \in S_N$ }
          \State $r \minuseq \lambda_F {\cdot} (s^\prime.N_A - s^\prime.N_B)$ 
          \State \hspace{0.5in} $\cdot(\hat{p}_B - \hat{p}_A)/N$
        \EndIf
        \State $r \minuseq \lambda_K$
      \State \Return $r$
     \EndFunction
     \end{algorithmic}
    %\end{algorithm}
    \end{minipage}
    \endgroup
    
    \caption{\Ourmethod{} algorithm pseudocode. The algorithm populates tables U and A with optimal utilities and actions, respectively. 
    Tables U and A are indexed by states; i.e., U[$s$] yields the utility for state $s$. 
    The for-loop on line 5 iterates through states in order of decreasing $\underline{T}$.
    The for-loop on line 7 iterates through all possible actions for the current state;
    and the loop on line 9 computes the expectation of $U$ for the current state and action.
    Function $R$ evaluates the reward function given by Equation \ref{eq:reward}.}
    \label{fig:pseudocode}
\end{figure}

\begin{figure}
    \centering
    \begin{minipage}{0.35\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/history_rar.png}\\
    \includegraphics[width=\textwidth]{figures/history_blockrar.png}
    \end{minipage}%
    \begin{minipage}{0.64\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/history_blockraropt_fc4_bc01.png}
    \end{minipage}\\
    \hspace{1.0in} (A) \hfill (B) \hspace{2.0in}
    \caption{Simulated trial histories. 
             Each plot traces the treatment allocation of 10,000 simulated trials.
             Histograms on the right give distributions of final allocations and report the mean.
             For each of these plots, $(p_A,p_B){=}(0.4, 0.1)$.
             (A) Histories for RAR and blocked RAR trial designs.
             (B) Histories for a \Ourmethod{} design, with parameter settings $\lambda_F{=}4.0$ and $\lambda_K{=}0.01$.
             Under these settings our algorithm allocates many more patients on average to the superior treatment.
             }
    \label{fig:histories}
\end{figure}

\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
    \input{figures/table_alt_fc04_bc01}
    }
    \caption{Simulation study alternative scenarios.
             Labels RAR, BRAR, and MDP refer to adaptive trials designed by RAR, blocked RAR, and \Ourmethod{}, respectively.
             \Ourmethod{} used parameter settings $\lambda_F{=}4.0$ and $\lambda_K{=}0.01$.
             The multicolumns marked as ``$Z$-scores'' report gain relative to the traditional 1:1 trial design, computed as $Z{=}(\mu_1 - \mu_2)/\sqrt{(\sigma_1^2 + \sigma_2^2)/10{,}000}$.
             With these particular parameter settings our algorithm attains lower power than the other designs, but its superior patient outcomes give it the greatest utility across all scenarios.}
    \label{tab:alt_table}
\end{table}

\begin{table}[]
    \centering
    \resizebox{0.8\textwidth}{!}{
    \input{figures/table_null_fc04_bc01}
    }
    \caption{Simulation study null scenarios. 
             Our algorithm produces designs with somewhat inflated Type-I error.
             This table excludes $F(h)$, which is always 0 since $p_A{=}p_B$.
             A 1:1 design is optimal under the null hypothesis; hence every adaptive design reports a relative decrease in utility.
             As in Table \ref{tab:alt_table}, these results use $\lambda_F{=}4.0$ and $\lambda_K{=}0.01$.}
    \label{tab:null_table}
\end{table}

\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/frontier_pa04_pb01_bc01.png}
    \includegraphics[scale=0.45]{figures/frontier_pa07_pb04_bc01.png}\\[-1em]
    (A) \hspace{2.5in} (B)
    \caption{Frontier plots. 
    Trial designs are shown as points in two dimensions, with statistical power on the horizontal axis and allocation to $A$ on the vertical axis---higher and to the right is better.
    As we vary $\lambda_F$ our algorithm traces a frontier in this space.
    (A) In this case ($p_A{=}0.4, p_B{=}0.1$) \Ourmethod{} dominates the other adaptive designs when $\lambda_F{=}2$; it attains higher power \emph{and} allocation to the superior treatment.
    (B) In other cases (e.g., $p_A{=}0.7, p_B{=}0.4$) \Ourmethod{} does not dominate the other designs, but gives a richer set of tradeoffs between power and patient outcomes.
    In both plots $\lambda_F{\in}\{2,3,4,5\}$ and $\lambda_K{=}0.01$.
    }
    \label{fig:frontiers}
\end{figure}

\begin{table}[]
    \centering
    \input{figures/redesign_table}
    \caption{Results of trial redesign. 
             Running our algorithm with $\lambda_F{=}3.0$, $\lambda_K{=}0.05$ yielded a trial design with Type-I error of 0.055 under the null, and power 0.557 under the alternative.
             Compare with a power of ${\sim}0.61$ for a traditional trial.
             The last two columns show the 10\%-ile and 90\%-ile of $N_A{-}N_B$.
             Notice that the design had probability ${<}10\%$ of assigning more patients to the inferior treatment.}
    \label{tab:redesign}
\end{table}
